Prevention and control of Zika fever as a mosquito-borne and sexually transmitted disease

The ongoing Zika virus (ZIKV) epidemic poses a major global public health emergency. It is known that ZIKV is spread by \textit{Aedes} mosquitoes, recent studies show that ZIKV can also be transmitted via sexual contact and cases of sexually transmitted ZIKV have been confirmed in the U.S., France, and Italy. How sexual transmission affects the spread and control of ZIKV infection is not well-understood. We presented a mathematical model to investigate the impact of mosquito-borne and sexual transmission on spread and control of ZIKV and used the model to fit the ZIKV data in Brazil, Colombia, and El Salvador. Based on the estimated parameter values, we calculated the median and confidence interval of the basic reproduction number R0=2.055 (95% CI: 0.523-6.300), in which the distribution of the percentage of contribution by sexual transmission is 3.044 (95% CI: 0.123-45.73). Our study indicates that R0 is most sensitive to the biting rate and mortality rate of mosquitoes while sexual transmission increases the risk of infection and epidemic size and prolongs the outbreak. In order to prevent and control the transmission of ZIKV, it must be treated as not only a mosquito-borne disease but also a sexually transmitted disease.

==> fitting.tex <==
\begin{tabular}{c|cc} 
\hline
parameter & estimate & assumed range \\
\hline
$\rho$ & 0.012  & [0,1] \\
$\tau_1$ & 0.404  & [0,$\infty$]\\
$m_1$ &   0.001  & [0,20]\\
$m_2$ &   9.525  & [0,20]\\
$m_3$ &  13.100  & [0,20]\\
$m_4$ &   8.129  & [0,20]\\
$S_{h,\text{Brazil}}$ &    0.516  & [0.5,0.95]\\
$E_{h,\text{Brazil}}$ & 0.000657  & [9.79e-9,1]\\
$I_{h1,\text{Brazil}}$ & 0.000657  & $\equiv E_{h,\text{Brazil}}$ \\
$I_{h2,\text{Brazil}}$ & 0.000657  & $\equiv E_{h,\text{Brazil}}$ \\
$A_{h,\text{Brazil}}$ & 0.000657  & $\equiv E_{h,\text{Brazil}}$ \\
$S_{v,\text{Brazil}}$ &  & 1-2e-4\\
$E_{v,\text{Brazil}}$ &  & 1e-4\\
$I_{v,\text{Brazil}}$ &  & 1e-4 \\
$S_{h,\text{Colombia}}$ &    0.705  & [0.5,0.95]\\
$E_{h,\text{Colombia}}$ & 2.515e-07  & [4.27e-8, 2.13e-7]\\
$I_{h1,\text{Colombia}}$ & 2.515e-07  & $\equiv E_{h,\text{Colombia}}$ \\
$I_{h2,\text{Colombia}}$ & 2.515e-07  & $\equiv E_{h,\text{Colombia}}$ \\
$A_{h,\text{Colombia}}$ & 2.515e-07  & $\equiv E_{h,\text{Colombia}}$ \\
$S_{v,\text{Colombia}}$ &   & 1-2e8\\
$E_{v,\text{Colombia}}$ &   & 1e-8 \\
$I_{v,\text{Colombia}}$ &   & 1e-8 \\
$S_{h,\text{El Salvador}}$ &    0.647  & [0.5, 0.95]\\
$E_{h,\text{El Salvador}}$ & 8.076e-07  & [3.25e-7, 1.628e-6]\\
$I_{h1,\text{El Salvador}}$ & 8.076e-07  & $\equiv E_{h,\text{El Salvador}}$ \\
$I_{h2,\text{El Salvador}}$ & 8.076e-07  & $\equiv E_{h,\text{El Salvador}}$ \\
$A_{h,\text{El Salvador}}$ & 8.076e-07  & $\equiv E_{h,\text{El Salvador}}$ \\
$S_{v,\text{El Salvador}}$ &   & 1-2e-8\\
$E_{v,\text{El Salvador}}$ &   & 1e-8\\
$I_{v,\text{El Salvador}}$ &   & 1e-8 \\
\hline
\end{tabular}

